A critical analysis of self-supervision, or what we can learn from a single image

We look critically at popular self-supervision techniques for learning deep convolutional neural networks without manual labels. We show that three different and representative methods, BiGAN, RotNet and DeepCluster, can learn the first few layers of a convolutional network from a single image as well as using millions of images and manual labels, provided that strong data augmentation is used. However, for deeper layers the gap with manual supervision cannot be closed even if millions of unlabelled images are used for training. We conclude that: (1) the weights of the early layers of deep networks contain limited information about the statistics of natural images, that (2) such low-level statistics can be learned through self-supervision just as well as through strong supervision, and that (3) the low-level statistics can be captured via synthetic transformations instead of using a large image dataset.

==> fig-conv-and-filterviz.tex <==
\begin{figure}[!tb]
\centering
\begin{minipage}{.40\textwidth}
\begin{tabular}{lccc}
\toprule
& \multicolumn{3}{c}{Method} \\
\cmidrule(l){2-4}
  & BiGAN& RotNet& DeepCluster\\
\midrule
{\rotatebox[origin=t]{90}{\qquad  via Image \texttt{A}}}&
\includegraphics[width=1.5cm]{figs/ameyoko_bigan.png}&
\includegraphics[width=1.5cm]{figs/RotNet_ameyoko_mono_ep80.png}&
\includegraphics[width=1.5cm]{figs/DC_ameyoko_mono.png}\\[-9mm]
 &20.4 & 19.9 & 20.7\\[+1mm]
{\rotatebox[origin=t]{90}{\qquad  via Image \texttt{B}}} &
\includegraphics[width=1.5cm]{figs/BiGAN_animals_d35_sc4000_16_full112max_wsF_upTrue_2o5M.png}&
\includegraphics[width=1.5cm]{figs/rotnet_animals.png} &
\includegraphics[width=1.5cm]{figs/DC_anim_conv1.png} \\[-9mm]
&20.5 &17.8 & 19.7\\
\bottomrule
\end{tabular}
\caption{\textbf{\texttt{conv1} filters trained using a single image.} The 
96 learned $(3 \! \times \! 11 \! \times \! 11)$ filters for the first layer of AlexNet are shown for each single training image and method along with their linear classifier performance. For visualization, each filter is normalized to be in the range of $(-1,1)$.}
\label{fig:conv1-comparison}
\end{minipage}
\begin{minipage}{.46\textwidth}
\centering
\includegraphics[width=0.93\linewidth]{figs/actmax_and_retrieval_both_largergap.png}
\caption{\textbf{Filter visualization.} We show activation maximization (left) and retrieval of top 9 activated images from the training set of ImageNet (right) for four random non-cherrypicked target filters. From top to bottom: \texttt{conv1-5} of the BiGAN trained on a single image \texttt{A}. The filter visualization is obtained by learning a (regularized) input image that maximizes the response to the target filter using the library Lucid \citep{olah2018building}.
\label{fig:actmax}}

\end{minipage}
\end{figure}

==> tab-linear-cifar10.tex <==
\begin{table}[t]
\centering
\caption{\textbf{CIFAR-10.} Accuracy of linear classifiers on features extracted at different depths of the network. %
}\label{tab:linprobes:cifar10}
\begin{tabular}{lrrrr} 
\toprule
  & \multicolumn{4}{c}{CIFAR-10} \\
  & \texttt{conv1} & \texttt{conv2} & \texttt{conv3} & \texttt{conv4} \\ \midrule
Fully supervised & $66.5$ & $70.1$ & $72.4$ & $75.9$  \\ 
Random & $57.8$ & $55.5$ & $54.2$ & $47.3$  \\ 
\midrule 
RotNet & $64.4$ & $65.6$ & $65.6$ & $59.1$  \\ 
GAN (CIFAR-10) & $67.7$ & $\mathbf{73.0}$ & $\mathbf{72.5}$ & $\textbf{69.2}$  \\ 
MonoGAN & $\mathbf{68.1}$ & $72.3$ & $70.8$ & $63.5$ \\
\bottomrule
\end{tabular}
\end{table}

==> tab-linear-cifar100.tex <==
\begin{table}[t]
\centering
\caption{\textbf{CIFAR-100.} Accuracy of linear classifiers on features extracted at different depths of the network.}\label{tab:linprobes:cifar100}
\begin{tabular}{lrrrr}
\toprule
  & \multicolumn{4}{c}{CIFAR-100} \\
  & \texttt{conv1} & \texttt{conv2} & \texttt{conv3} & \texttt{conv4} \\ \midrule
Fully supervised & $38.7$ & $43.6$ & $44.4$ & $46.5$  \\ 
Random & $30.9$ & $29.8$ & $28.6$ & $24.1$  \\ 
\midrule
RotNet & $36.0$ & $35.9$ & $34.2$ & $25.8$  \\ 
GAN (CIFAR-100) &  $38.1$ &  $42.2$ & $44.0$ & $\mathbf{46.6}$ \\
GAN (CIFAR-10) & $39.6$ & $46.0$ & $\mathbf{45.1}$ & $39.9$  \\ 
MonoGAN & $\mathbf{39.9}$& $\mathbf{46.9}$ & $44.5$ & $38.8$  \\ 	
\bottomrule
\end{tabular}
\end{table}

==> tab-linear.tex <==
\setlength{\tabcolsep}{2pt}
\begin{table*}[!ht]
\centering
\caption{
  \textbf{ImageNet LSVRC-12 linear probing evaluation.} A linear classifier is trained on the (downsampled) activations of each layer in the pretrained model.
  We report classification accuracy averaged over $10$ crops.
  The $^\ddagger$ indicated that numbers are taken from \citep{Zhang17} .
}
\small
  \begin{tabular}{cl r l rrrrr}
    \toprule
          &&~~~& \multicolumn{5}{c}{ILSVRC-12} \\
    &Method, Reference & \#images & & \texttt{conv1} & \texttt{conv2} & \texttt{conv3} & \texttt{conv4} & \texttt{conv5} \\
    \midrule
    (a)&Full-supervision$^\ddagger$                        &$1,\!281,\!167$&  & $19.3$ & $36.3$ & $44.2$ & $48.3$ & $50.5$     \\
    (b)&\citep{oyallon2017scaling}: Scattering &0 &&-& $18.9$ & - & - & -\\
    (c)&Random$^\ddagger$                     &0&  & $11.6$ & $17.1$ & $16.9$ & $16.3$ & $14.1$    \\
    (d)&\citep{krahenbuhl16}:$k$-means$^\ddagger$     &$\approx \! 160$&  & $17.5$ & $23.0$ & $24.5$ & $23.2$ & $20.6$ \\
    \midrule
    (e)&\citep{Donahue17}: BiGAN$^\ddagger$      &$1,\!281,\!167$&  & $17.7$ & $24.5$ & $31.0$ & $29.9$ & $28.0$    \\
    (f)&\quad mono, Image \texttt{A} &$1$&    &  $20.4$ & $30.9$ & $33.4$ & $28.4$ & $16.0$   \\
    (g)&\quad mono, Image \texttt{B} &$1$&    &  $20.5$ & $30.4$ & $31.6$ & $27.0$ & $16.8$   \\
    (h)&\quad deka                   &$10$&   & $16.2$ & $16.5$ & $16.5$ & $13.1$ & $7.5$  \\
    (i)&\quad kilo                   &$1,\!000$& & $16.1$ & $17.7$ & $18.3$ & $17.6$ & $13.5$ \\
    \midrule
    (j)&\citep{Gidaris18}: RotNet      &$1,\!281,\!167$&  & $18.8$ & $31.7$ & $38.7$&  $38.2$ & $36.5$ \\
    (k)&\quad mono, Image \texttt{A}  &$1$&   & $19.9$ & $30.2$ & $30.6$ & $27.6$ & $21.9$  \\
    (l)&\quad mono, Image \texttt{B}  &$1$&   & $17.8$ & $27.6$ & $27.9$ & $25.4$ & $20.2$  \\
    (m)&\quad deka                    &$10$&  & $19.6$ & $30.7$ & $32.6$ & $28.9$ & $22.6$  \\
    (n)&\quad kilo                    &$1,\!000$&& $21.0$ & $33.5$ & $36.5$ & $34.0$ & $29.4$  \\
    \midrule
    (o)&\citep{Caron18}: DeepCluster &$1,\!281,\!167$&  & $18.0$ & $32.5$ &  $39.2$ & $37.2$ &  $30.6$ \\ %
    (p)&\quad mono, Image \texttt{A} &$1$&   & $20.7$ & $31.5$ & $32.5$ & $28.5$ & $21.0$ \\
    (q)&\quad mono, Image \texttt{B} &$1$&   & $19.7$ & $30.1$ & $31.6$ & $28.5$ & $20.4$ \\
    (s)&\quad deka                   &$10$&  & $18.5$ & $29.0$ & $31.1$ & $28.2$ & $21.9$\\
    (t)&\quad kilo                   &$1,\!000$&& $19.5$ & $29.8$ & $33.0$ & $31.7$ & $26.8$\\
    \bottomrule
  \end{tabular}
\label{tab:linear}
\end{table*}
